Understanding the Effects of AI-Assisted Critical Thinking on Human-AI Decision Making

Despite the growing prevalence of human-AI decision making, the human-AI team's decision performance often remains suboptimal, partially due to insufficient examination of humans' own reasoning. In this paper, we explore designing AI systems that directly analyze humans' decision rationales and encourage critical reflection of their own decisions. We introduce the AI-Assisted Critical Thinking (AACT) framework, which leverages a domain-specific AI model's counterfactual analysis of human decision to help decision-makers identify potential flaws in their decision argument and support the correction of them. Through a case study on house price prediction, we find that AACT outperforms traditional AI-based decision-support in reducing over-reliance on AI, though also triggering higher cognitive load. Subgroup analysis reveals AACT can be particularly beneficial for some decision-makers such as those very familiar with AI technologies. We conclude by discussing the practical implications of our findings, use cases and design choices of AACT, and considerations for using AI to facilitate critical thinking.

==> figs/algo_full.tex <==

\begin{algorithm}[t!]
\caption{AI-Assisted Critical Thinking: full workflow. } 
\label{alg:full}
\small
\begin{algorithmic}[1]
\REQUIRE $x = \{X_1=v_1 \ldots X_n=v_n\}$: Test instance
\REQUIRE $P_m(y | \boldsymbol{\cdot})$: Probability function from AI
\REQUIRE $\epsilon\in[0,1]$: feature importance threshold
\STATE Initialize $\boldsymbol{x_h}, y_h, p_h \gets get\_DM\_args(\boldsymbol{x})$
\STATE Initialize $F \gets \emptyset$ 
\WHILE {$True$}
    \STATE // \textbf{Critique Support}
    \STATE $F \gets \emptyset$ 
    \FOR {$X_i\in x_h$}
        \IF { $P_m(y_h|\boldsymbol{x_h}) - P_m(y_h|\boldsymbol{x_h} - \{X_i=v_i\}) > \epsilon$}
        \STATE $F \gets F \cup \{X_i\}$  // $get\_support\_features$
        \ENDIF
    \ENDFOR
    \STATE \textit{prompt\_reflection(F)}   
    \STATE \textit{present\_features(F)}    
    \STATE \textit{get\_data\_probability(F)}   
    \STATE $\boldsymbol{x_h}, y_h, p_h \gets check\_update(\boldsymbol{x})$  
    \STATE // \textbf{Critique Incompleteness}
    \STATE $F \gets \emptyset$ 
    \FOR {$X_i\notin x_h$}
        \IF {$P_m(y_h|\boldsymbol{x_h}\cup \{X_i=v_i\}) - P_m(y_h|\boldsymbol{x_h}) > \epsilon$}
        \STATE $F \gets F \cup \{X_i\}$   // $get\_missing\_features$
        \ENDIF
    \ENDFOR
    \STATE \textit{prompt\_reflection(F)}   
    \STATE \textit{present\_features(F)}    
    \STATE \textit{get\_data\_probability(F)}   
    \STATE $\boldsymbol{x_h}, y_h, p_h \gets check\_update(\boldsymbol{x})$  
    \IF{$check\_stopping()=True$}
        \STATE break
    \ENDIF
    \STATE // \textbf{Critique Unreliability}
    \STATE $F \gets \emptyset$ 
    \FOR {$X_i\notin x_h$}
        \IF {$|P_m(y_h|\boldsymbol{x_h}-\{X_i=v_i\})-P_m(y_h|\boldsymbol{x_h})|\leq\epsilon$}
        \STATE $F \gets F \cup \{X_i\}$   // $get\_irrelevant\_features$
        \ELSIF {$P_m(y_h|\boldsymbol{x_h}-\{X_i=v_i\}) - P_m(y_h|\boldsymbol{x_h}) > \epsilon$}
        \STATE $F \gets F \cup \{X_i\}$   // $get\_opposing\_features$
        \ENDIF
    \ENDFOR
    \STATE \textit{prompt\_reflection(F)}   
    \STATE \textit{present\_features(F)}    
    \STATE \textit{get\_data\_probability(F)}   
    \STATE $\boldsymbol{x_h}, y_h, p_h \gets check\_update(\boldsymbol{x})$  
    \IF{$check\_stopping()=True$}
        \STATE break
    \ENDIF
    \STATE // \textbf{Critique Conflict}   
    \STATE $F \gets \emptyset$ 
    \FOR {$y_c\neq y_h$}
        \STATE $\boldsymbol{x_c^*}= \arg\max_{\boldsymbol{x_c}\subseteq\boldsymbol{x_i}} P_m(y_c|\boldsymbol{x_c})$
        \STATE $F \gets F \cup \{(x_c^*, y_c, P_m(y_c|\boldsymbol{x_c^*} )\}$   // $get\_conflicting\_arguments$
    \ENDFOR
    \STATE \textit{prompt\_reflection(F)}   
    \STATE \textit{present\_features(F)}    
    \STATE \textit{get\_data\_probability(F)}   
    \STATE $\boldsymbol{x_h}, y_h, p_h \gets check\_update(\boldsymbol{x})$  
    \IF{$check\_stopping()=True$}
        \STATE break
    \ENDIF
\ENDWHILE
\STATE  \textbf{return} $y_h$
\end{algorithmic} 
\end{algorithm}

% \begin{algorithm}[t!]
% \caption{AI-Assisted Critical Thinking: example workflow} 
% \label{alg:workflow}
% \small
% \begin{algorithmic}[1]
% \STATE \textbf{input}: test case $\boldsymbol{x}\in X_{test}$
% \STATE $\boldsymbol{x_h}, y_h, p_h=get\_DM\_args(\boldsymbol{x})$
% \STATE  $F=get\_supporting\_features(\boldsymbol{x_h}, y_h)$
% \STATE  $prompt\_reflect(F)$
% \STATE  present $F$
% \STATE  present $get\_data\_probability(F)$
% \STATE $//$ \textbf{Critiquing Incompleteness}
% \STATE  $F=get\_missing\_features(\boldsymbol{x_h}, y_h)$
% \STATE  $prompt\_reflect(F)$
% \STATE  present $F$
% \STATE  present $get\_data\_probability(F)$
% \STATE  $\boldsymbol{x_h}, y_h, p_h = check\_update()$
% \STATE  $check\_stopping(p_h)$
% \STATE $//$ \textbf{Critiquing Unreliability}
% \STATE  $F=get\_irrelevant\_features(\boldsymbol{x_h}, y_h)$
% \STATE  $prompt\_reflect(F)$
% \STATE  present $F$
% \STATE  present $get\_data\_probability(F)$
% \STATE  $F=get\_opposing\_features(\boldsymbol{x_h}, y_h)$
% \STATE  $prompt\_reflect(F)$
% \STATE  present $F$
% \STATE  present $get\_data\_probability(F)$
% \STATE  $\boldsymbol{x_h}, y_h, p_h = check\_update()$
% \STATE  $check\_stopping(p_h)$
% \STATE $//$ \textbf{Critiquing Conflict}
% \STATE  $C=get\_conflicting\_arguments(y_h)$
% \STATE  $prompt\_reflect(C)$
% \STATE  present $C$
% \STATE  present $get\_data\_probability(C)$
% \STATE  $\boldsymbol{x_h}, y_h, p_h = check\_update()$
% \STATE  \textbf{return} $\boldsymbol{x_h}, y_h, p_h$
% \end{algorithmic} 
% \end{algorithm}


% \begin{algorithm}[t!]
% \caption{AACT Example: Critique-Correction-Update cycle for Incompletness}
% \label{alg:aact}
% \begin{algorithmic}[1]
% \REQUIRE $x = \{X_1=v_1 \ldots X_n=v_n\}$: Test instance
% \REQUIRE $x_h \subseteq x$: DM's arguments, $y_h$: DM's hypothesis, $p_h\in[0,1]$: DM's confidence
% \REQUIRE $P_m(y | x)$: Probability function from AI
% \REQUIRE $\epsilon$: feature importance threshold
% \STATE // Find features DM may have missed (\textit{get\_missing\_features(x\_h, y\_h)})
% \STATE Initialize $F \gets \emptyset$ 
%     \FOR {$X_i\notin x_h$}
%         \IF {$P_m(y_h|\boldsymbol{x_h}\cup \{X_i=v_i\}) - P_m(y_h|\boldsymbol{x_h}) > \epsilon$}
%         \STATE $F \gets F \cup \{X_i\}$
%         \ENDIF
%     \ENDFOR
% \STATE Prompt DM to reflect on features in F // \textit{prompt\_reflection(F)}
% \STATE Present features in F as missing features // \textit{present\_features(F)}
% \STATE Present data probability for features in F //\textit{data\_probability(F)}
% \STATE Check if DM wants to update arguments // \textit{check\_update()}
% \STATE Check stopping condition // \textit{check\_stopping()}
% \STATE \textbf{Return} $y_h$
% \end{algorithmic}
% \end{algorithm}


==> figs/algo_short.tex <==

\begin{algorithm}[t!]
\caption{AI-Assisted Critical Thinking: shortened example workflow (full workflow in Appendix~\ref{app:workflow}). } 
\label{alg:short}
\small
\begin{algorithmic}[1]
\Require $x = \{X_1=v_1 \ldots X_n=v_n\}$: Test instance
\Require $P_m(y | \boldsymbol{\cdot})$: Probability function from AI
\Require $\epsilon\in[0,1]$: feature importance threshold
\State Initialize $\boldsymbol{x_h}, y_h, p_h \gets get\_DM\_args(\boldsymbol{x})$
\State Initialize $F \gets \emptyset$ 
\While {$True$}
    \State // \textbf{Critique Support}
    \State \ldots
    % \FOR {$X_i\in x_h$}
    %     \IF { $P_m(y_h|\boldsymbol{x_h}) - P_m(y_h|\boldsymbol{x_h} - \{X_i=v_i\}) > \epsilon$}
    %     \State $F \gets F \cup \{X_i\}$  \\ $get\_support\_features$
    %     \ENDIF
    % \ENDFOR
    \State // \textbf{Critique Incompleteness}
    \State $F \gets \emptyset$ 
    \For {$X_i\notin x_h$}
        \If {$P_m(y_h|\boldsymbol{x_h}\cup \{X_i=v_i\}) - P_m(y_h|\boldsymbol{x_h}) > \epsilon$}
        \State $F \gets F \cup \{X_i\}$   // $get\_missing\_features$
        \EndIf
    \EndFor
    \State \textit{prompt\_reflection(F)}   
    \State \textit{present\_features(F)}    
    \State \textit{get\_data\_probability(F)}   
    \State $\boldsymbol{x_h}, y_h, p_h \gets check\_update(\boldsymbol{x})$  
    \If{$check\_stopping()=True$}
        \State break
    \EndIf
    \State // \textbf{Critique Unreliability}
    \State \ldots
    \State // \textbf{Critique Conflict}    
    \State \ldots
\EndWhile
\State  \textbf{return} $y_h$
\end{algorithmic} 
\end{algorithm}


==> tables/demo.tex <==
\begin{table}[b!]
\centering
\small
\caption{Demographics survey questions, excluding education.\textbf{*} indicated questions with reverse scoring.}
\label{table:demo}

\begin{tabular}{p{0.25\linewidth}p{0.7\linewidth}}
\toprule
\textbf{Category} & \textbf{Questions} \\
\midrule

\multirow{4}{*}{Need for Cognition (NFC)} &
I would prefer complex to simple problems.\\
\cmidrule(l){2-2}
& I like to have the responsibility of handling a situation that requires a lot of thinking.\\
\cmidrule(l){2-2}
& \textbf{*}Thinking is \textbf{not} my idea of fun.\\
\cmidrule(l){2-2}
& \textbf{*}I would rather do something that requires little thought than something that is sure to challenge my thinking abilities.\\
\midrule

AI Familiarity &
How familiar are you with artificial intelligence (AI) technologies?\\
\midrule

Task Familiarity &
How familiar are you with the task background of real estate markets?\\
\midrule

\multirow{3}{*}{Cognitive Reflection Test (CRT)} &
A bat and a ball cost \$1.10 in total. The bat costs \$1.00 more than the ball. How much does the ball cost?\\
\cmidrule(l){2-2}
& If it takes 5 machines 5 minutes to make 5 widgets, how long would it take 100 machines to make 100 widgets?\\
\cmidrule(l){2-2}
& In a lake, there is a patch of lily pads. Every day, the patch doubles in size. If it takes 48 days for the patch to cover the entire lake, how long would it take for the patch to cover half of the lake?\\
\bottomrule
\end{tabular}
\end{table}

